Adversarial Training of Self-supervised Monocular Depth Estimation against Physical-World Attacks

Monocular Depth Estimation (MDE) is a critical component in applications such as autonomous driving. There are various attacks against MDE networks. These attacks, especially the physical ones, pose a great threat to the security of such systems. Traditional adversarial training method requires ground-truth labels hence cannot be directly applied to self-supervised MDE that does not have ground-truth depth. Some self-supervised model hardening techniques (e.g., contrastive learning) ignore the domain knowledge of MDE and can hardly achieve optimal performance. In this work, we propose a novel adversarial training method for self-supervised MDE models based on view synthesis without using ground-truth depth. We improve adversarial robustness against physical-world attacks using L0-norm-bounded perturbation in training. We compare our method with supervised learning based and contrastive learning based methods that are tailored for MDE. Results on two representative MDE networks show that we achieve better robustness against various adversarial attacks with nearly no benign performance degradation.

==> MDE_Model_Hardening (ICLR 2023) (Camera Ready, Arxiv Full2)/Conclusion.tex <==
\vspace{-10pt}
\section{Conclusion}
\vspace{-7pt}
We tackle the problem of hardening self-supervised Monocular Depth Estimation (MDE) models against physical-world attacks without using the depth ground truth. We propose a self-supervised adversarial training method  using view synthesis considering camera poses and use $L_0$-norm-bounded perturbation generation in training to improve physical-world attacks robustness. Compared with traditional supervised learning-based and contrastive learning-based methods, our method achieves better robustness against various adversarial attacks in both the digital world and the physical world with nearly no benign performance degradation. 

==> MDE_Model_Hardening (ICLR 2023) (Camera Ready, Arxiv Full2)/Evaluation.tex <==
\vspace{-5pt}
\section{Evaluation}\label{sec:eval}
\vspace{-5pt}
In this section, we evaluate the performance of our method in white-box, black-box, and physical-world attack scenarios, and discuss the ablations. Our code is available at: \url{https://github.com/Bob-cheng/DepthModelHardening}
\vspace{-7pt}
\subsection{Experimental Setup.}\label{sec:ES}
\vspace{-7pt}
\textbf{Networks and Dataset.} We$_{\!}$ use$_{\!}$ Monodepth2~\citep{monodepth2}$_{\!}$ and$_{\!}$ DepthHints~\citep{watson2019self}$_{\!}$ as$_{\!}$ our$_{\!}$ subject$_{\!}$ networks$_{\!}$ to$_{\!}$ harden.$_{\!}$ They$_{\!}$ are$_{\!}$ representative$_{\!}$ and$_{\!}$ popular$_{\!}$ self-supervised$_{\!}$ MDE$_{\!}$ models$_{\!}$ that$_{\!}$ are$_{\!}$ widely$_{\!}$ used$_{\!}$ as$_{\!}$ benchmarks$_{\!}$ in$_{\!}$ the$_{\!}$ literature.$_{\!}$ Both$_{\!}$ models$_{\!}$ are$_{\!}$ trained$_{\!}$ on$_{\!}$ the$_{\!}$ KITTI$_{\!}$ dataset~\citep{Geiger2013IJRR}$_{\!}$ and$_{\!}$ our$_{\!}$ methods fine-tune$_{\!}$ the$_{\!}$ original$_{\!}$ models publicly available. 

\begin{table}[t]
    \centering
    \vspace{-10pt}
    \caption{\small \textbf{Benign performance} of original and hardened models on depth estimation. }
    \label{tab:ben_perf}
    \vspace{-5pt}
    \scalebox{0.72}{
    \begin{threeparttable}
    \begin{tabular}{lcccccccccc}
\toprule
  & \multicolumn{5}{c}{Monodepth2} & \multicolumn{5}{c}{DepthHints} \\ \cline{2-11} Models
 & ABSE$\downarrow$ & RMSE$\downarrow$ & ABSR$\downarrow$ & SQR$\downarrow$ & $\delta\uparrow$ & ABSE$\downarrow$ & RMSE$\downarrow$ & ABSR$\downarrow$ & SQR$\downarrow$ & $\delta\uparrow$ \\ \midrule\midrule
Original & 2.125 & 4.631 & 0.106 & 0.807 & 0.877 & 2.021 & 4.471 & 0.100 & 0.728 & 0.886 \\
L0+SelfSup (Ours) & 2.16 & 4.819 & 0.105 & 0.831 & 0.874 & 2.123 & 4.689 & 0.103 & 0.777 & 0.877 \\
L0+Sup & 2.162 & 4.648 & 0.110 & 0.846 & 0.876 & 2.015 & 4.453 & 0.100 & 0.734 & 0.887 \\
L0+Contras & 3.218 & 6.372 & 0.155 & 1.467 & 0.782 & 3.626 & 6.742 & 0.209 & 1.561 & 0.694 \\
PGD+SelfSup & 2.169 & 4.818 & 0.105 & 0.826 & 0.874 & 2.120 & 4.680 & 0.103 & 0.774 & 0.877 \\
PGD+Sup & 2.153 & 4.637 & 0.109 & 0.838 & 0.876 & 2.019 & 4.460 & 0.101 & 0.736 & 0.886 \\
PGD+Contras & 3.217 & 6.083 & 0.194 & 1.825 & 0.756 & 3.928 & 7.526 & 0.213 & 2.256 & 0.701 \\ \bottomrule
\end{tabular}
\begin{tablenotes}
    \item  * \added{For hardened models, A+B denotes generating adversarial perturbation with method A and training with method B.}
\end{tablenotes}
\end{threeparttable}
}

\vspace{-10pt}
\end{table}

\textbf{Baselines.} There$_{\!}$ are$_{\!}$ no$_{\!}$ direct baselines$_{\!}$ available$_{\!}$ since$_{\!}$ no$_{\!}$ prior$_{\!}$ works$_{\!}$ have$_{\!}$ been focusing on hardening MDE models as far as we know. Hence we extend state-of-the-art contrastive learning-based and supervised learning-based adversarial training methods to MDE  and use them as our baselines. They do not require ground-truth depth, same as our self-supervised method. Details are in 
Appendix~\ref{app:baseline}

\textbf{Training Setup.} In adversarial training, the ranges of distance $z_c$ and viewing angle $\alpha$ are sampled randomly from 5 to 10 meters and -30 to 30 degrees, respectively. The view synthesis uses EoT~\citep{athalye2018synthesizing}. We generate the adversarial perturbations with two methods:$_{\!}$ $L_0$-norm-bounded$_{\!}$ with$_{\!}$ $\epsilon_{\!}=_{\!}1/10$ and $L_\infty$-norm-bounded ($i.e.,$ PGD~\citep{madry2018towards}) with $\epsilon_{\!}=_{\!}0.1$. The latter is for comparison purposes. 
We train with our self-supervised method and two baseline methods based on contrastive learning and supervised learning. Hence, there are 6 approaches combining the 2 perturbation generation methods with the 3 training methods. With these approaches, we fine-tune the original model for 3 epochs on the KITTI dataset and produce 6 hardened models for each network. Other detailed configurations and the selection of 2D object images are in 
Appendix~\ref{app:training_config}.

\textbf{Attacks.} We conduct various kinds of attacks to evaluate the robustness of different models. They are $L_0$-norm-bounded attacks with $\epsilon=1/20, 1/10, 1/5 \text{ and } 1/3$, $L_\infty$-norm-bounded (PGD) attacks with $\epsilon=0.05, 0.1 \text{ and } 0.2$ (image data are normalized to [0,1]), and an adversarial patch attack in \citet{mathew2020monocular}. Adversarial perturbation or patch is applied to an object image. The patch covers 1/10 of the object at the center. Each attack is evaluated with 100 randomly selected background scenes. The object is placed at a distance range of 5 to 30 meters and a viewing angle range of -30 to 30 degrees. We report the average attack performance over different background scenes, distances, and viewing angles for each attack. In addition, we conduct the state-of-the-art physical-world attack \citep{cheng2022physical} with the printed optimal patch and a real vehicle in driving scenarios. Adversarial examples are in 
Appendix~\ref{append:adv_egs}. \added{Evaluation with more attacks are in Appendix~\ref{app:more_atks}}.

\textbf{Metrics.} We use the mean absolute error (ABSE), root mean square error (RMSE), relative absolute error (ABSR), relative square error (SQR), and the ratio of relative absolute error under 1.25 ($\delta$) 
as the evaluation metrics. These metrics are widely used in evaluating depth estimation performance. Metric $\delta$  denotes the percentage of pixels of which the ratio between the estimated depth and ground-truth depth is smaller than 1.25.
It is the higher, the better and the others are the lower, the better. The definition of each metric can be found in 
Appendix~\ref{app:eval_metrics}.




\vspace{-5pt}
\subsection{Main Results}\label{sec:main_results}
\vspace{-5pt}

\textbf{Benign Performance. }  Together with the original model, we have 7 models under test for each network. We evaluate the depth estimation performance on the KITTI dataset using the Eigen split and report the results in Table~\ref{tab:ben_perf}. 
As shown, self-supervised and supervised methods have little influence on the models' depth estimation performance, which means these approaches can harden the model with nearly no benign performance degradation. In contrast, the contrastive learning-based approach performs the worst. The ABSE of estimated depth is over 1 m worse than the original model. The reason could be that contrastive learning itself does not consider the specific task ($i.e.,$ MDE) but fine-tunes the encoder to filter out the adversarial perturbations. Thus the benign performance is sacrificed during training. The other two methods consider the depth estimation performance either by preserving the geometric relationship of 3D space in synthesized frames or by supervising the training with estimated depth.



\begin{table}[t]
    \centering
    \vspace{-12pt}
    \caption{\small \textbf{Defence performance} of original and hardened models under attacks.}
    \label{tab:attack_perf}
    \vspace{-5pt}
    \scalebox{0.71}{
    \begin{threeparttable}
    \begin{tabular}{clcccccccccccccc}
\toprule
 & \multirow{2}{*}{Attacks} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{\makecell{L0+SelfSup\\(Ours)}} & \multicolumn{2}{c}{L0+Sup} & \multicolumn{2}{c}{L0+Contras} & \multicolumn{2}{c}{PGD+SelfSup} & \multicolumn{2}{c}{PGD+Sup} & \multicolumn{2}{c}{PGD+Contras} \\ \cline{3-16} 
 &  & \small{ABSE}$\downarrow$ & $\delta\uparrow$ & \small{ABSE}$\downarrow$ & $\delta\uparrow$ & \small{ABSE}$\downarrow$ & $\delta\uparrow$ & \small{ABSE}$\downarrow$ & $\delta\uparrow$ & \small{ABSE}$\downarrow$ & $\delta\uparrow$ & \small{ABSE}$\downarrow$ & $\delta\uparrow$ & \small{ABSE}$\downarrow$ & $\delta\uparrow$ \\ \midrule\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{Monodepth2}} 
 & L0 1/20 & 4.71 & 0.65 & \textbf{0.18} & \textbf{0.99} &\underline{ 0.44 }& \underline{0.98} & 1.30 & 0.67 & 0.49 & 0.95 & 0.58 & 0.94 & 0.69 & 0.94 \\
 & L0 1/10 & 6.08 & 0.51 & \textbf{0.25} & \textbf{0.98} & {0.94} & \underline{0.93} & 1.75 & 0.54 & \underline{0.82} & 0.91 & 1.18 & 0.79 & 0.96 & 0.89 \\
 & L0 1/5 & 8.83 & 0.39 & \textbf{0.34 }& \textbf{0.9 }& {1.59} & \underline{0.85} & 2.32 & 0.46 & 2.33 & 0.70 & 2.72 & 0.51 & \underline{1.11} & {0.85} \\
 & L0 1/3 & 9.99 & 0.34 &\textbf{ 0.52} &\textbf{ 0.96} & {2.08} & \underline{0.78} & 2.65 & 0.41 & 4.32 & 0.51 & 4.09 & 0.41 & \underline{1.75} & 0.70 \\
 & PGD 0.05 & 4.74 & 0.56 & \underline{0.82} & \underline{0.97} & 1.29 & 0.80 & 6.61 & 0.38 & \textbf{0.67 }& \textbf{0.98 }& 0.82 & 0.95 & 1.82 & 0.67 \\
 & PGD 0.1 & 11.68 & 0.34 & \underline{1.53} & \underline{0.85} & 2.53 & 0.71 & 12.74 & 0.24 & \textbf{1.38} & \textbf{0.95 }& 1.64 & 0.76 & 2.66 & 0.53 \\
 & PGD 0.2 & 17.10 & 0.23 & \textbf{3.46} & \textbf{0.69} & 6.14 & 0.50 & 20.14 & 0.15 & \underline{3.81} & \underline{0.58} & 5.04 & 0.32 & 3.97 & 0.42 \\
 & Patch & 2.71 & 0.77 & \textbf{0.39} & \textbf{0.98} & 1.35 & 0.89 & 6.40 & 0.52 & \underline{0.40} & \underline{0.98} & 0.84 & 0.92 & 0.50 & 0.95 \\ \hline
\multirow{8}{*}{\rotatebox[origin=c]{90}{DepthHints}}
 & L0 1/20 & 2.33 & 0.66 &\textbf{ 0.19} & \textbf{0.99} & 0.34 & 0.96 & 1.06 & 0.83 & \underline{0.22} & \underline{0.99} & 0.58 & 0.89 & 0.40 & 0.99 \\
 & L0 1/10 & 3.19 & 0.59 &\textbf{ 0.27} & \textbf{0.99} & 0.48 & 0.95 & 1.56 & 0.77 & \underline{0.42} & \underline{0.98} & 1.03 & 0.79 & 0.60 & 0.97 \\
 & L0 1/5 & 4.77 & 0.42 & \textbf{0.40} & \textbf{0.98} & 0.96 & 0.82 & 1.85 & 0.75 & 0.83 & 0.92 & 1.93 & 0.68 & \underline{0.66} & \underline{0.95}  \\
 & L0 1/3 & 6.03 & 0.36 &\textbf{ 0.48} & \textbf{0.98} & 1.64 & 0.68 & 2.60 & 0.69 & 1.45 & 0.79 & 3.06 & 0.57 & \underline{1.16} & \underline{0.82} \\
 & PGD 0.05 & 3.11 & 0.48 & \textbf{0.62 }& \textbf{0.98} & 1.23 & 0.75 & 4.05 & 0.55 & \underline{0.64} & \underline{0.98} & 0.93 & 0.79 & 1.16 & 0.79 \\
 & PGD 0.1 & 6.44 & 0.36 & \underline{1.27} & \underline{0.86} & 2.37 & 0.62 & 7.59 & 0.36 &\textbf{ 1.21 }& \textbf{0.92 }& 1.76 & 0.67 & 1.74 & 0.62  \\
 & PGD 0.2 & 18.37 & 0.23 & \underline{3.09} & \underline{0.60} & 7.13 & 0.41 & 13.59 & 0.24 & 6.14 & \textbf{0.68} & 4.22 & 0.37 & \textbf{2.60} & 0.49 \\
 & Patch & 0.70 & 0.91 & 0.46 & 0.95 & 0.53 & 0.93 & 6.90 & 0.49 & 0.46 & 0.95 & \underline{0.36} & \textbf{0.99} & \textbf{0.34} & \underline{0.98} \\ \bottomrule
\end{tabular}
\begin{tablenotes}
\item *Bold and underlining indicate the best and second best performance in each row. \added{Hardened models are named the same as Table 1.}
\end{tablenotes}
\end{threeparttable}
}
\vspace{-17pt}
\end{table}




\textbf{White-box Attacks.} We conduct various white-box attacks on each model to evaluate the robustness of hardened models. Specifically, for each model, we compare the estimated depth of the adversarial scene ($i.e.,$ $I_{t}'$) with that of the corresponding benign scene ($i.e.,$ $I_{t}$ in Equation~\ref{eq:it_syn}) and larger difference means worse defense performance. Table~\ref{tab:attack_perf} shows the result. As shown, all the hardened models have better robustness than the original models against all kinds of attacks, and it is generic on the two representative MED networks, which validates the effectiveness of our adversarial training approaches. Comparing different approaches, \texttt{L0+SelfSup} has the best performance in general. It reduces the ABSE caused by all-level $L_0$-norm-bounded attacks from over 4.7~m to less than 0.6~m. Specifically,$_{\!}$ the$_{\!}$ self-supervision-based$_{\!}$ method$_{\!}$ outperforms$_{\!}$ the$_{\!}$ contrastive$_{\!}$ learning-based$_{\!}$ and$_{\!}$ the$_{\!}$ supervision-based$_{\!}$ methods$_{\!}$ regardless$_{\!}$ of$_{\!}$ the$_{\!}$ perturbation$_{\!}$ generation$_{\!}$ method$_{\!}$ used. It is because the self-supervision-based method follows the original training procedure that is carefully designed for the network and has been evaluated thoroughly. It is not$_{\!}$ surprising$_{\!}$ that$_{\!}$ models$_{\!}$ adversarially$_{\!}$ trained$_{\!}$ with$_{\!}$ $L_0$-norm-bounded$_{\!}$ perturbation$_{\!}$ (our$_{\!}$ method)$_{\!}$ achieve better robustness against $L_0$-norm-bounded attacks and so do PGD-based methods, but more importantly, $L_0$-norm-based training also has good defense performance against PGD attacks. The robustness of \texttt{L0+SelfSup} is only slightly worse than \texttt{PGD+SelfSup} on some PGD attacks and even better than it on stronger PGD attacks. An explanation is that $L_0$-norm does not restrict the magnitude of perturbation on each pixel, and stronger PGD attacks are closer to this setting ($i.e.,$ high-magnitude perturbations) and can be well-defended using the $L_0$-norm-based adversarial training. Monodepth2 is vulnerable to the patch attack, and this kind of attack can be well-defended by our methods. \texttt{L0+SelfSup} also performs the best. Depthhints itself is relatively robust to the patch attack, and our methods can further reduce the attack effect. Our defense generalizes well to complex scenes including  various road types, driving speed, and the density of surrounding objects. Qualitative results are in Appendix~\ref{append:adv_egs}.


\setlength{\intextsep}{0pt}
\begin{wraptable}{r}{0.59\textwidth}
    \centering
    \caption{\small Defence performance of original and hardened models under\textbf{ black-box attacks}. }
    \label{tab:black_box}
    \vspace{-5pt}
    \scalebox{0.71}{
    \begin{threeparttable}
    \begin{tabular}{lcccccccc}
\toprule
\multicolumn{1}{r}{Target} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{\makecell{L0+SelfSup\\(Ours)}} & \multicolumn{2}{c}{L0+Sup} & \multicolumn{2}{c}{L0+Contras} \\ \cline{2-9} 
Source & ABSE & $\delta\uparrow$ &ABSE & $\delta\uparrow$ & ABSE & $\delta\uparrow$& ABSE & $\delta\uparrow$\\ \midrule\midrule
Original & - & - & \textbf{0.25} & \textbf{0.99} & 0.55 & 0.95 & 1.35 & 0.71 \\
L0+SelfSup & \textbf{0.52} & \textbf{0.93} & - & - & \textbf{0.24} & \textbf{0.98} & \textbf{0.45} & \textbf{0.95} \\
L0+Sup & 1.09 & 0.80 & \textbf{0.29} & \textbf{0.99} & - & - & 0.65 & 0.89 \\
L0+Contras & 2.65 & 0.50 & \textbf{0.22} & \textbf{0.99} & 0.27 & 0.98 & - & - \\ \bottomrule
\end{tabular}
\begin{tablenotes}
\item *Bold indicates the best performance in each row or column.
\end{tablenotes}
\end{threeparttable}
}
\end{wraptable}
\textbf{Black-box Attacks.} We also validate our methods against black-box attacks.$_{\!}$ We$_{\!}$ use$_{\!}$ the$_{\!}$ original$_{\!}$ Monodepth2 model$_{\!}$ and the models fine-tuned with $L_0$-norm-bounded perturbations and the three training methods. We perform $L_0$-norm-bounded attacks on each model with $\epsilon=1/10$ and apply the generated adversarial object to other models evaluating the black-box attack performance.$_{\!}$ The$_{\!}$ first$_{\!}$ column$_{\!}$ in$_{\!}$ Table~\ref{tab:black_box}$_{\!}$ denotes$_{\!}$ the$_{\!}$ source$_{\!}$ models$_{\!}$ and$_{\!}$ other$_{\!}$ columns$_{\!}$ are the target models' defense performance.$_{\!}$ Looking at each column,  adversarial examples generated from \texttt{L0+SelfSup} have the worst attack performance, which indicates the low transferability of adversarial examples generated from the model trained with our self-supervised methods. From each row, we can observe that \texttt{L0+SelfSup} has the best defense performance against adversarial examples generated from each$_{\!}$ source$_{\!}$ model, which$_{\!}$ further validates the robustness of \texttt{L0+SelfSup}. In summary,$_{\!}$ the$_{\!}$ self-supervised$_{\!}$ training$_{\!}$ method$_{\!}$ can$_{\!}$ produce$_{\!}$ safer$_{\!}$ and$_{\!}$ more$_{\!}$ robust$_{\!}$ models.$_{\!}$ Their$_{\!}$ adversarial$_{\!}$ examples$_{\!}$ have low transferability and they defend against black-box attacks well.


\begin{figure}
\centering
\vspace{-5pt}
\begin{minipage}{.27\textwidth}
 \centering
    \includegraphics[width=\textwidth]{Figs/physical2.png}
    \caption{\small Physical-world attack and defence. Video: {\footnotesize \url{https://youtu.be/_b7E4yUFB-g}}}
    \label{fig:physical_atk}
\end{minipage}%
\hfill
\begin{minipage}{.7\textwidth}
  \centering
    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{Figs/distance_L0.pdf}
        \caption{\small $L_0$-norm attack. }
        \label{fig:attack_dist_l0}
    \end{subfigure}
    \hspace{5pt}
    \begin{subfigure}[t]{0.45\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{Figs/distance_PGD.pdf}
        \caption{\small PGD and patch attack. }
        \label{fig:attack_dist_pgd}
    \end{subfigure}   
\caption{\small Robustness with different \textbf{training distance ranges}.}\label{fig:attack_dist}
\end{minipage}
\vspace{-15pt}
\end{figure}

\textbf{Physical-world Attacks.}  Our evaluation with the state-of-the-art physical-world MDE attack~\citep{cheng2022physical} validates the effectiveness of our method in various real-world lighting conditions, driving operations, road types, etc. The experimental settings are the same as \citet{cheng2022physical}. Figure~\ref{fig:physical_atk} shows the result. The first row is the real-world adversarial scene, in which a car is moving with an adversarial patch attached to the rear. The second row is the depth predicted by the original Monodepth2 model and the third row is predicted by our hardened model (\texttt{L0+SelfSup}). The ``hole'' in the output of the original model caused by the adversarial patch is fixed in our hardened model. It is known that the adversarial attacks designed for the physical world are still generated in the digital world and they have better digital-world attack performance than physical-world performance because additional environmental variations in the physical world degrade the effectiveness of adversarial patterns~\citep{braunegg2020apricot,wu2020making,cheng2022physical}. Hence, defending attacks in the digital world is more difficult and our success in digital-world defense in previous experiments has implied effectiveness in the physical world.


\vspace{-5pt}
\subsection{Ablations}
\vspace{-5pt}

\textbf{Distance Range in Training.} While synthesizing views in training, the range of distance $z_c$ of the target object is randomly sampled from $d_1$ to $d_2$ meters. In this ablation study, we evaluate the effect of using different ranges of distance in training. We use  \texttt{L0+SelfSup} to fine-tune the original Monodepth2 model. 
The ranges of distance we use in training are [5, 5], [5, 10], [5, 15], [5, 20], [5, 25] and [5, 30] (Unit: meter). 
Note that, for a fair comparison, the range of distance we use in model evaluation is always from 5 to 30 meters. The results are shown in Figure~\ref{fig:attack_dist}. As shown, the model trained with a distance range of 5-10 meters has the best robustness and a larger or smaller distance range could lead to worse performance. It is because further distances lead to smaller objects on the image and fewer pixels are affected by the attack. Thus the attack performance is worse at further distances and training with these adversarial examples is not the most effective. If the distance in training is too small ($e.g.,$ 5 meters), the model cannot defend various scales of attack patterns and cannot generalize well to further distances. In our experiments, the range of 5-10 meters makes a good balance between training effectiveness and generality. 

Other ablation studies about viewing angles range in training are in Appendix~\ref{app:ang_range}, transferability to unseen target objects is in Appendix~\ref{append:target_objs}, comparing training from scratch and fine-tuning is in 
Appendix~\ref{app:scratch}
and the performance of method combinations can be found in 
Appendix~\ref{app:combi}.



==> MDE_Model_Hardening (ICLR 2023) (Camera Ready, Arxiv Full2)/Introduction.tex <==
\vspace{-10pt}
\section{Introduction}\label{sec:intro}
\vspace{-5pt}


Monocular Depth Estimation (MDE) is a technique that estimates depth from a single image. 
It enables 2D-to-3D projection by predicting the depth value for each pixel in a 2D image and serves as a very affordable replacement for the expensive Lidar sensors.
It hence has a wide range of applications such as autonomous driving~\citep{tesla-self-supervised}, visual SLAM~\citep{wimbauer2020monorec}, and visual relocalization~\citep{lm-reloc-2020}, etc. In particular, self-supervised MDE gains fast-growing popularity  in the industry ($e.g.,$ Tesla Autopilot~\citep{tesla-self-supervised}) because it does not require the ground-truth depth collected by Lidar during training while achieving comparable accuracy with supervised training.
Exploiting vulnerabilities of deep neural networks, multiple digital-world~\citep{zhang2020adversarial,wong2020targeted} and physical-world attacks~\citep{cheng2022physical} against MDE have been proposed. They mainly use optimization-based methods to generate adversarial examples to fool the MDE network.  Due to the importance and broad usage of self-supervised MDE, these$_{\!}$ adversarial$_{\!}$ attacks$_{\!}$ have$_{\!}$ posed$_{\!}$ a$_{\!}$ great$_{\!}$ threat$_{\!}$ to$_{\!}$ the$_{\!}$ security$_{\!}$ of$_{\!}$ applications$_{\!}$ such$_{\!}$ as$_{\!}$ autonomous$_{\!}$ driving,$_{\!}$ which$_{\!}$ makes$_{\!}$ the$_{\!}$ defense$_{\!}$ and$_{\!}$ MDE model$_{\!}$ hardening$_{\!}$ an urgent need. 



Adversarial training \citep{goodfellow2014explaining} is the most popular and effective way to defend adversarial attacks.$_{\!}$ However,$_{\!}$ it$_{\!}$ usually$_{\!}$ requires$_{\!}$ ground$_{\!}$ truth$_{\!}$ labels$_{\!}$ in$_{\!}$ training, making it not directly applicable to self-supervised MDE models with no depth ground truth.
Although contrastive learning gains a lot of attention recently and has been used for self-supervised adversarial training~\citep{ho2020contrastive,kim2020adversarial}, it does not consider$_{\!}$ the$_{\!}$ domain$_{\!}$ knowledge$_{\!}$ of$_{\!}$ depth estimation and can hardly achieve optimal results (shown in Section~\ref{sec:main_results}).
In addition, many existing adversarial training methods do not consider certain properties of physical-world attacks such as strong perturbations. Hence in this paper, we focus on addressing the problem of \textit{hardening self-supervised MDE models against physical-world attacks without requiring the ground-truth depth.}

A straightforward proposal to harden MDE models is to perturb 3D objects in various scenes and ensure the estimated depths remain correct. However, it is difficult to realize such adversarial training. First, 3D perturbations are difficult to achieve in the physical world. While one can train the model in simulation, such training needs to be supported by a high-fidelity simulator and a powerful scene rendering engine that can precisely project 3D perturbations to 2D variations. Second, since self-supervised MDE training does not have the ground-truth depth, even if realistic 3D perturbations could be achieved and used in training, the model may converge on incorrect (but robust) depth estimations. In this paper, we propose a new self-supervised adversarial training method for MDE models.
Figure~\ref{fig:intro} provides a conceptual illustration of our technique. A board $A$ 
printed with the 2D image of a 3D object ($e.g.,$ a car) is placed at a fixed location (next to the car at the top-right corner). 
We use two cameras (close to each other at the bottom) $C_t$ and $C_s$ %\xz{annotate $C$ and $C'$} 
to provide a stereo view of the board (images $I_t$ and $I_s$ in Figure~\ref{fig:2d_frames}). 
Observe that there are fixed geometric relations between pixels in the two 2D views produced by the two respective cameras such that the image in one view can be transformed to yield the image from the other view. 
\added{Intuitively, $I_t$ can be acquired by shifting $I_s$ to the right}.
Note that when two cameras are not available, one can use two close-by frames in a video stream to form the two views as well. 
During adversarial training, camera $C_t$ takes a picture $I_t$ of the original 2D image board $A$. Similarly, camera $C_s$ takes a picture $I_s$ of the board too (step \ding{182}). The bounding box of the board $A$ is recognized in $I_t$ and the pixels in the bounding box corresponding to $A$ are perturbed (step \ding{183}). 
Note that these are 2D perturbations similar to those in traditional adversarial training. 
At step \ding{184}, the perturbed image $I_t$+perturbations is fed to the MDE model to make depth estimation, achieving a 3D projection of the object. 
Due to the perturbations, a vulnerable model generates distance errors as denoted by the red arrow between $A$ and the projected 3D object in Figure~\ref{fig:intro}. 
At step \ding{185}, we try to reconstruct $I_t$ from $I_s$. The reconstruction is parameterized on the cameras' relative pose transformations and the estimated distance of the object from the camera. Due to the distance error, the reconstructed image $I_{s\rightarrow t}$ (shown in Figure~\ref{fig:2d_frames}) is different from $I_t$. Observe that part of the car (the upper part inside the red circle) is distorted. In comparison, Figure~\ref{fig:2d_frames} also shows the reconstructed image $I^{ben}_{s\rightarrow t}$ without the perturbation, which is much more similar to $I_t$. The goal of our training (of the subject MDE model) is hence to reduce the differences between$_{\!}$ original$_{\!}$ and$_{\!}$ reconstructed$_{\!}$ images.$_{\!}$ The$_{\!}$ above$_{\!}$ process$_{\!}$ is$_{\!}$ conceptual,$_{\!}$ whose$_{\!}$ faithful$_{\!}$ realization$_{\!}$ entails$_{\!}$ a substantial physical-world overhead. In Section~\ref{sec:methods}, 
we describe how to avoid the majority of the physical-world cost through image synthesis and training on synthesized data. 

\added{While traditional adversarial training
%~\citep{goodfellow2014explaining,moosavi2016deepfool,madry2018towards} 
assumes bounded perturbations in $L_2$ or $L_{\infty}$ norm (i.e., measuring the overall perturbation magnitude on all pixels), physical-world attacks are usually unbounded in those norms. 
They tend to be stronger attacks in order to be persistent with environmental condition variations. To harden MDE models against such attacks, we utilize a loss function that can effectively approximate the $L_0$ norm (measuring the number of perturbed pixels regardless of their perturbation magnitude) while remaining differentiable. Adversarial samples generated by minimizing this loss can effectively mimic physical attacks. We make the following contributions:}



\begin{figure}
     \centering
     \begin{subfigure}[b]{0.77\textwidth}
         \centering
        \includegraphics[width=\textwidth]{Figs/intro_3D.png}
        \caption{\small Conceptual illustration. }
        \label{fig:intro}
     \end{subfigure}
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
      \includegraphics[width=\textwidth]{Figs/large_frames.png}
      \caption{\small Different Views.
      }
      \label{fig:2d_frames}
     \end{subfigure}
     \vspace{-20pt}
     \caption{\small Self-supervised adversarial training of MDE with view synthesis. }
     \label{fig:highlight_intro}
     \vspace{-15pt}
\end{figure}


\vspace{-7pt}
\begin{itemize}[leftmargin=10pt]
\setlength\itemsep{-2pt}

    \item We develop a new method to synthesize 2D images that follow physical-world constraints (e.g., relative camera positions) and directly perturb such images in adversarial training. The physical world cost is hence minimized.
  \item Our method utilizes {\em the reconstruction consistency} from one view to the other view to enable self-supervised adversarial training without the ground-truth depth labels.
  \item \added{We$_{\!}$ generate $L_0$-bounded perturbations$_{\!}$ with$_{\!}$ a$_{\!}$ differentiable$_{\!}$ loss$_{\!}$ and$_{\!}$ randomize$_{\!}$ the$_{\!}$ camera$_{\!}$ and$_{\!}$ object$_{\!}$ settings$_{\!}$ during$_{\!}$ synthesis$_{\!}$ to$_{\!}$ effectively$_{\!}$ mimic$_{\!}$ physical-world$_{\!}$ attacks$_{\!}$ and$_{\!}$ improve$_{\!}$ robustness.}

  
 \item We evaluate the method and compare it with a supervised learning baseline and a contrastive learning baseline, adapted from  state-of-the-art adversarial contrastive learning~\citep{kim2020adversarial}. Results show that our method achieves better robustness against various adversarial attacks with nearly no model performance degradation. The average depth estimation error of an adversarial object with 1/10 area of perturbation is reduced from 6.08 m to 0.25 m by our method, better than 1.18 m by the supervised learning baseline. Moreover, the contrastive learning baseline degrades model performance a lot. Our physical-world experiments video is available at \url{https://youtu.be/_b7E4yUFB-g}.

  
\end{itemize}



==> MDE_Model_Hardening (ICLR 2023) (Camera Ready, Arxiv Full2)/Method.tex <==
\vspace{-7pt}
\section{Our Design}\label{sec:methods}
\vspace{-5pt}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{Figs/object_def_proj.png}
    \caption{\small (a) Bird view of the relative positions of the camera and the target object. (b) 3D coordinates of the four corners of the object in the camera frame. (c) Projection from the physical-world object to the two views.}\label{fig:synth_def}
    %\xz{change $u_0$ to $u^t_0$ and $u'_0$ to $u^s_0$ and the text accordingly. We need to use consistent symbols}}
    \vspace{-15pt}
\end{figure}
 
Our technique consists of a few components.
The first one (Section~\ref{sec:view_syn}) is view synthesis that generates the two views $I_t$ and $I_s$ of the object  and is equivalent to
step \ding{182} in Figure~\ref{fig:intro}. 
The second one (Section~\ref{sec:adv_perturb}) is robust adversarial perturbation that perturbs $I_t$ to induce maximum distance errors (step \ding{183} in Figure~\ref{fig:intro}).
The third one (Section~\ref{sec:MDE_training}) is the self-supervised adversarial training (steps \ding{184} and \ding{185}). We will discuss the details of these components and then present the training pipeline at the end. 




\vspace{-10pt}
\subsection{View Synthesis To Avoid Physical World Scene Mutation}\label{sec:view_syn}
\vspace{-5pt}
As mentioned in Section~\ref{sec:intro},  conceptually we need to place an image board of the 3D object at some physical locations on streets and use two cameras to take pictures of the board. In order to achieve robustness in training, we ought to vary the image of the object (e.g., different cars), the position of the image board, the positions and angles of the cameras, and the street view.
This entails enormous overhead in the physical world.
Therefore, we propose a novel view synthesis technique that requires minimal physical world overhead. Instead, it directly synthesizes $I_s$ and $I_t$ with an object in some street view, reflecting different settings of the aforementioned configurations. 

Specifically, we use one camera to take a picture $I_t$ of a 2D image board $A$ of the object, with the physical width and height $W$ and $H$, respectively. 
As shown in Figure~\ref{fig:synth_def} (b), the four corners of the board have the 3D coordinates ($x^t_0$, $y^t_0$, $z^t_0$), ..., and ($x^t_3$, $y^t_3$, $z^t_3$), respectively, in the camera frame, namely, the coordinate system with the camera as the origin.
The camera is placed at $z_c$ distance away from the board with an angle of $\alpha$, as shown in Figure~\ref{fig:synth_def} (a).
The size of the board is true to the rear of the object. This is important for the later realistic synthesis step.

After that, we derive a projection function that can map a pixel in $A$ to a pixel in $I_t$. The function is parameterized on $W$, $H$, $z_c$, $\alpha$, etc. such that {\em we can directly use it to synthesize a large number of $I_t$'s with different $A$'s by changing those parameter settings.} To acquire $I_s$ that is supposed to form a stereo view with $I_t$, we do not necessarily need another camera in the physical world. Instead, we can use two neighboring video frames of some street view ($e.g.,$ from the KITTI dataset~\citep{Geiger2013IJRR}), denoted as $R_t$ and $R_s$, to approximate a stereo pair taken by two close-by cameras.
Note that the differences between the two images implicitly encode the relative positions of the two cameras. 
A prominent benefit of such approximation is that a large number of camera placements and street views can be easily approximated by selecting various neighboring video frames. This is consistent with existing works~\citep{monodepth2,watson2019self}. 
We replace the area in $I_t$ that does not correspond to $A$, i.e., the background of the object, with the corresponding area in $R_t$. Intuitively, we acquire a realistic $I_t$ by stamping the object's image to a background image. The synthesis respects physical world constraints.
A projection function parameterized by $R_t$ and $R_s$ can be derived to map a pixel in one camera's view to a pixel in the other.
Then, we project the part of $I_t$ that corresponds to $A$ using the projection function and stamp it on $R_s$, acquiring $I_s$. As such, the resulted view of $A$ (in $I_s$) is consistent with the camera pose denoted by $R_s$.
$I_t$ and $I_s$ are then used in model hardening (discussed later in Section~\ref{sec:MDE_training}).

Formally, if the center of the physical camera's view aligns with the center of the image board $A$, the correlation between a pixel ($u^A,v^A$) in $A$ and its 3D coordinate ($x^t$, $y^t$, $z^t$)  is:
\begin{gather}\label{eq:img2board}
\scalebox{1}{$
    \begin{aligned}
        \begin{bmatrix}
            x^t\\y^t\\z^t\\1
        \end{bmatrix} = 
        \begin{bmatrix}
            \cos\alpha & 0 & -\sin\alpha & 0\\
            0 & 1 & 0 & 0\\
            \sin\alpha & 0 & \cos\alpha & z_c \\
            0 & 0 & 0 & 1
        \end{bmatrix}\cdot
        \begin{bmatrix}
            W/w & 0 & -W/2\\
            0 & H/h & -H/2\\
            0 & 0 & 0\\
            0 & 0 & 1
        \end{bmatrix}\cdot
        \begin{bmatrix}
            u^A \\ v^A \\ 1
        \end{bmatrix},
    \end{aligned}
$}
\end{gather}
where $w$ and $h$ are the width and height of $A$ in pixels. The other variables ($e.g., \alpha, z_c, W, H, etc.$) are defined in Figure~\ref{fig:synth_def}.
The 3D coordinates can be further projected 
to pixels in $I_t$ and $I_s$ as: 

\begin{gather}\label{eq:pixel_proj}
    \begin{aligned}
        \begin{bmatrix}
            u^t~v^t~1
        \end{bmatrix}^\top &= 1/z^t\cdot K\cdot 
        \begin{bmatrix}
            x^t~y^t~z^t~1
        \end{bmatrix}^\top,\\
        \begin{bmatrix}
            u^s~v^s~1
        \end{bmatrix}^\top &= 1/{z^s}\cdot K \cdot
        \begin{bmatrix}
            x^s~y^s~z^s~1
        \end{bmatrix}^\top, \ \ \ 
        \begin{bmatrix}
            x^s~y^s~z^s~1
        \end{bmatrix}^\top = T_{t\rightarrow s} \cdot\begin{bmatrix}
            x^t~y^t~z^t~1
        \end{bmatrix}^\top,
    \end{aligned}
\end{gather}
where $T_{t\rightarrow s}$ is {\em the camera pose transformation} (CPT) that projects 3D coordinates in the physical camera $C_t$'s coordinate system to coordinates in the other (virtual) camera $C_s$'s  coordinate system. It is determined by $R_s$ and $R_t$ as mentioned before. 
$K$ is the camera intrinsic.
Combining Equation~\ref{eq:img2board} and Equation~\ref{eq:pixel_proj}, we know the projections from pixel $(u^A, v^A)$ of the object image to pixel $(u^t, v^t)$ in $I_t$ and to pixel $(u^s, v^s)$ in $I_s$. 
Let     $\begin{bmatrix}
            u^t~v^t~1
        \end{bmatrix}^\top = P^{A\rightarrow t}_{z_c, \alpha}(u^A, v^A)$ and $\begin{bmatrix}
            u^s~v^s~1
        \end{bmatrix}^\top = P^{A\rightarrow s}_{z_c, \alpha, T_{t\rightarrow s} }(u^A, v^A)$.
We synthesize $I_t$ and $I_s$ as:
\begin{gather}
\begin{aligned}\label{eq:it_syn}
    I_t[u,v]=\left\{ 
        \begin{aligned}
          A[u^A,v^A],  & \qquad \begin{bmatrix}
            u~v~1
        \end{bmatrix}^\top = P^{A\rightarrow t}_{z_c, \alpha}(u^A, v^A) \\
        R_t[u,v],  & \qquad \qquad \qquad otherwise
        \end{aligned}\right.,
\end{aligned}
\end{gather}
\begin{gather}
\begin{aligned}\label{eq:is_syn}
    \quad \ \ \ I_s[u,v]=\left\{
        \begin{aligned}
          A[u^A,v^A],  & \qquad \begin{bmatrix}
            u~v~1
        \end{bmatrix}^\top = P^{A\rightarrow s}_{z_c, \alpha, T_{t\rightarrow s} }(u^A, v^A) \\
        R_s[u,v],  & \qquad \qquad \qquad otherwise
        \end{aligned}\right.,
\end{aligned}
\end{gather}
where $R_t$ and $R_s$ are the background images implicitly encoding the camera relative poses.
A large number of $I_t$ and $I_s$ are synthesized by varying $R_t$, $R_s$, $z_c$, $\alpha$, $A$, and used in hardening. The creation induces almost zero cost compared to creating a physical world dataset with similar diversity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\vspace{-5pt}
\subsection{Robust Adversarial Perturbations}\label{sec:adv_perturb}
\vspace{-5pt}
We use an optimization based method to generate robust adversarial perturbations $\delta$ on the object image $A$ composing the corresponding adversarial object $A+\delta$ and synthesize $I'_t$ by replacing $A$ with  $A+\delta$ in Equation~\ref{eq:it_syn}.
The synthesized $I'_t$ is then used in adversarial training. We bound the perturbations with $L_0$-norm, which is to constrain the number of perturbed pixels. Compared with digital-world attacks that use traditional $L_\infty$-norm or $L_2$-norm-bounded perturbations ($e.g.,$ FGSM~\citep{goodfellow2014explaining}, Deepfool~\citep{moosavi2016deepfool},  and PGD~\citep{madry2018towards}), physical-world attacks usually use adversarial patches ~\citep{brown2017adversarial} without restrictions on the magnitude of perturbations in the patch area because stronger perturbations are needed to induce persistent model misbehavior in the presence of varying environmental conditions ($e.g.,$ lighting conditions, viewing angles, distance and camera noise). Hence, $L_0$-norm is more suitable in physical-world attacks because it restricts the number of pixels to perturb without bounding the perturbation magnitude of individual pixels. However, the calculation of $L_0$-norm is not differentiable by definition and hence not amenable for optimization. We hence use a soft version of it as proposed in ~\citet{Tao2022BetterTrigger}. The main idea is to decompose the perturbations into positive and negative components and use the long-tail effects of $\tanh$ function, in the normalization term, to model the two ends of a pixel's value change ($i.e.,$ zero perturbation or arbitrarily large perturbation). As such, a pixel tends to have very large perturbation or no perturbation at all. 
\begin{align}
    \delta =& ~maxp \cdot (\texttt{clip}(b_p, 0, 1) - \texttt{clip}(b_n, 0, 1))  \label{eq:perturb}.\\ 
    \mathcal{L}_{pixel} =& \sum\limits_{h, w}\left(\max_c\left(\frac{1}{2}(\tanh(\frac{b_p}{\gamma}) + 1)\right)\right) +  \sum\limits_{h, w}\left(\max_c\left(\frac{1}{2}(\tanh(\frac{b_n}{\gamma}) + 1)\right)\right). \label{eq:perturb_norm}
\end{align}
Specifically, the perturbation is defined in Equation~\ref{eq:perturb} and the normalization term is $\mathcal{L}_{pixel}$ in Equation~\ref{eq:perturb_norm}, where $b_p$ and $b_n$ are the positive and negative components; \texttt{clip()} bounds the variable to a range of [0,1]; $h, w, c$ are the height, width and channels of image and $\gamma$ is a scaling factor. We refer readers to \citet{Tao2022BetterTrigger} for detailed explanations. 

Equation~\ref{eq:perturb_gen} gives the formal definition of our perturbation generation method,
where $S_{p}$ is a distribution of physical-world distance and view angles (e.g., reflecting the relations between cameras and cars during real-world driving); $S_R$ is the set of background scenes (e.g., various street views); $D()$ is the MDE model which outputs the estimated depth map of given scenario and $MSE()$ is the mean square error. 
\begin{gather}\label{eq:perturb_gen}
    \begin{aligned}
        \min\limits_{b_n, b_p} ~~& E_{z_c,\alpha\sim S_p, R_t \sim S_R}\left[MSE\left( D\left(I'_t\right)^{-1}, 0 \right)\right] + \mathcal{L}_{pixel}, \\ 
    s.t. ~~& L_0(\delta) \leq \epsilon.
    \end{aligned}
\end{gather}
Our adversarial goal is to make the target object further away, so we want to maximize the depth estimation ($i.e.,$ minimize the reciprocal). Intuitively, we synthesize $I'_t$ with random $R_t$ and different $\alpha$ and $z_c$ of object $A$ and use expectation of transformations (EoT) ~\citep{athalye2018synthesizing} to improve physical-world robustness. We minimize the mean square error between zero and the reciprocal of synthesized scenario's depth estimation in the adversarial loss term and use $\mathcal{L}_{pixel}$ as the normalization term of perturbations. Parameter $\epsilon$ is a predefined $L_0$-norm threshold of perturbations and it denotes the maximum ratio of pixels allowed to perturb ($e.g.,$ $\epsilon=1/10$ means 1/10 pixels can be perturbed at most).

\begin{figure}[t]
% \vspace{-10pt}
    \centering
        \includegraphics[width=0.85\textwidth]{Figs/training_pipeline.png}
        \caption{\small Pipeline of adversarial training of self-supervised monocular depth estimation. Solid lines denote data flow and dashed lines denote back propagation paths.
        }
        \label{fig:adv_training}
        \vspace{-10pt}
\end{figure}

\vspace{-5pt}
\subsection{Self-supervised MDE Training.}\label{sec:MDE_training}
\vspace{-5pt}
In each training iteration, we first synthesize $I_t$ and $I_s$ as mentioned earlier. Perturbations are then generated to $I_t$ to acquire $I'_t$ following Equation~\ref{eq:perturb_gen}.
As illustrated in Figure~\ref{fig:intro}, we reconstruct a version of $I_t$ from $I_s$ using the depth information derived from $I'_t$. We call the resulted image $I_{s\rightarrow t}$. Intuitively,  $I'_t$ causes depth errors which distort the
projection from $I_s$ to $I_{s\rightarrow t}$ such that the latter appears different from $I_t$. 
Similar to how we project ($u^A$, $v^A$) to ($u^t$, $v^t$) or ($u^s$, $v^s$) earlier in this section (i.e., Equation~\ref{eq:pixel_proj}), we can project ($u^s$, $v^s$) in $I_s$ to a pixel ($u^{s\rightarrow t}$, $v^{s\rightarrow t}$) in $I_{s\rightarrow t}$. This time, we use the depth information derived from $I'_t$. Formally, the projection is defined as:
\begin{gather}\label{eq:reconstruction}
    \begin{aligned}
        \begin{bmatrix}
            x^{s\rightarrow t}~y^{s\rightarrow t}~z^{s\rightarrow t}~1
        \end{bmatrix}^\top = K^{-1}\cdot D_{I'_t}(u^{s\rightarrow t},v^{s\rightarrow t}) \cdot \begin{bmatrix}
            u^{s\rightarrow t}~v^{s\rightarrow t}~1
        \end{bmatrix}^\top,\\ 
         \begin{bmatrix}
            x^s~y^s~z^s~1
        \end{bmatrix}^\top = T_{t\rightarrow s} \cdot \begin{bmatrix}
            x^{s\rightarrow t}~y^{s\rightarrow t}~z^{s\rightarrow t}~1
        \end{bmatrix}^\top,\ \ \ \ 
        \begin{bmatrix}
            u^s~v^s~1
        \end{bmatrix}^\top = 1/z^s\cdot K\cdot \begin{bmatrix}
            x^s~y^s~z^s~1
        \end{bmatrix}^\top.
    \end{aligned}
\end{gather}
Intuitively, there are relations between  2D image pixels and 3D coordinates, i.e., the first and the third formulas in Equation~\ref{eq:reconstruction}. 
The 3D coordinates also have correlations decided by camera poses, i.e., the second formula. Observe that, the first 2D-to-3D relation is parameterized on $D_{I'_t}$, the depth estimation of $I'_t$.
Let     $\begin{bmatrix}
            u^s~v^s
        \end{bmatrix}^\top = P_{D_{I'_t},T_{t\rightarrow s}}(u^{s\rightarrow t}, v^{s\rightarrow t})$
        be the transformation function that projects a pixel in $I_{s\rightarrow t}$ to a pixel in $I_s$ derived from Equation~\ref{eq:reconstruction}.
$I_{s\rightarrow t}$ is synthesized as:
\begin{gather}
    \begin{aligned}\label{eq:target_recons}
        I_{s\rightarrow t}[u, v] = I_s[ P_{D_{I'_t},T_{t\rightarrow s}}(u, v)].
    \end{aligned}
\end{gather}
Intuitively, it rearranges the pixels in $I_s$ to form $I_{s\rightarrow t}$. 
We then compare $I_{s\rightarrow t}$ with $I_t$ and minimize their difference to guide the training.

Our training pipeline is shown in Figure~\ref{fig:adv_training}. 
There are two trainable networks, the MDE model $D$ and a camera transposing model {\it TP}.
Recall that we need the camera pose transformation matrix $T_{t\rightarrow s}$ between the two cameras' coordinate systems. We hence train the {\it TP} network that predicts $T_{t\rightarrow s}$ from a given pair of background images $R_s$ and $R_t$. We denote it as: $T_{t\rightarrow s} = \textit{TP}(R_t, R_s)$.
Observe that in Figure~\ref{fig:adv_training}, from left to right, the pipeline takes the object image $A$ and synthesizes images $I_t$ and $I_s$.
$I_t$ and $A$ are further used to derive adversarial sample $I'_t$, which is fed to the depth network $D$ to acquire depth estimation. 
The depth information, the {\it TP} network's output $T_{t\rightarrow s}$, and $I_s$ are used to derive $I_{s\rightarrow t}$.
Two outputs $I_{s\rightarrow t}$ and $I_t$ are compared.
The training objective is hence as:
\begin{align}\label{eq:recons_loss}
    \min\limits_{\theta_{D}, \theta_{\textit{TP}}} \mathcal{L}_p &= pe(I_t, I_{s\rightarrow t}),
\end{align}
which is to update the weight values of $D$ and {\it TP} to minimize
the photometric reconstruction error of the two outputs, denoted by $pe()$. Specific designs of $pe()$ differ in literature but our model hardening technique is general to all self-supervised MDE methods.

==> MDE_Model_Hardening (ICLR 2023) (Camera Ready, Arxiv Full2)/Related_Works.tex <==

\vspace{-10pt}
\section{Related Works}
\vspace{-7pt}


\textbf{Self-supervised MDE.} Due to the advantage of training without the depth ground truth, self-supervised MDE has gained much attention recently. 
In such training, stereo image pairs and/or monocular videos are used as the training input. Basically, two images taken by camera(s) from adjacent poses are used in each optimization iteration.
A depth network and a pose network are used to estimate the depth map of one image
and the transformation between the two camera poses, respectively.
With the depth map and pose transformation, it further calculates the pixel correspondence across the images and then tries to rearrange the pixels in one image 
to reconstruct the other. The pose network and the depth network are updated simultaneously to minimize the reconstruction error. 
\citet{garg2016unsupervised} first propose to use color consistency loss between stereo images in training. \citet{zou2018df} enable video-based training with two networks (one depth network and one pose network). Many following works improve the self-supervision with new loss terms~\citep{godard2017unsupervised,bian2019unsupervised,wang2018learning,yin2018geonet,ramamonjisoa-2021-wavelet-monodepth,yang2020d3vo} or include temporal information~\citep{wang2019recurrent,zou2020learning,tiwari2020pseudo,watson2021temporal}. Among them, Monodepth2~\citep{monodepth2} significantly improves the performance with several novel designs such as minimum photometric loss selection, masking out static pixels, and multi-scale depth estimation. Depthhints~\citep{watson2019self} further improves it via additional depth suggestions obtained from stereo algorithms.  While such unsupervised training is effective, how to improve its robustness against physical attack remains an open problem.

\textbf{MDE Attack and Defense.} 
\citet{mathew2020monocular} use a deep feature annihilation loss to launch perturbation attack and patch attack. \citet{zhang2020adversarial} design a universal attack with a multi-task strategy and \citet{wong2020targeted} generate targeted adversarial perturbation on images which can alter the depth map arbitrarily. \citet{hu2019analysis} propose a defense method against perturbation attacks by masking out non-salient pixels. It requires another saliency prediction network. For physical-world attacks, \citet{cheng2022physical} generates a printable adversarial patch to make the vehicle disappear.
To the best of our knowledge, we are the first work focusing on improving the robustness of self-supervised MDE models against physical-world attacks.


\textbf{Adversarial Robustness.} It is known that deep neural networks (DNN) are vulnerable to adversarial attacks. Imperceptible input perturbations could lead to model misbehavior~\citep{szegedy2013intriguing,madry2018towards,moosavi2016deepfool}. Typically, adversarial training is used to improve the robustness of DNN models. It uses both benign and adversarial examples for training~\citep{madry2018towards,carlini2017towards,tramer2017ensemble}.
Adversarial training has been applied to many domains like image classification~\citep{carlini2017towards,madry2018towards}, object detection~\citep{zhang2019towards,chen2021robust,chen2021class}, and segmentation~\citep{xu2021dynamic,hung2018adversarial,arnab2018robustness} etc. A common requirement for adversarial training is supervision because generating adversarial examples needs ground truth, and most tasks require labels for training. Some semi-supervised adversarial learning methods~\citep{carmon2019unlabeled,alayrac2019labels} use a small portion of labeled data to enhance robustness. Contrastive learning~\citep{ho2020contrastive,kim2020adversarial} is also used with adversarial examples either for better self-supervised learning or to improve robustness. In this work, we explore the adversarial training of MDE without using ground-truth depth and compare our method with contrastive learning-based and supervised learning-based methods that are specifically tailored for MDE.
There are other defense techniques such as input transformations. However,
\citet{athalye2018obfuscated} point out that these techniques largely rely on obfuscated gradients which may not lead to true robustness. In the scenarios of autonomous driving, there are other works focusing on the security of Lidar or multi-sensor fusion-based systems~\citep{tu2020physically,tu2021exploring,cao2019adversarial,cao2021invisible}. They use sensor spoofing or adversarial shapes to fool the Lidar hardware or AI model, while in this work, we consider fully-vision-based autonomous driving systems in which MDE is the key component.



==> MDE_Model_Hardening (ICLR 2023) (Camera Ready, Arxiv Full2)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvi{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

